Self-Supervised Representation Learning for Astronomical Images

Sky surveys are the largest data generators in astronomy, making automated tools for extracting meaningful scientific information an absolute necessity. We show that, without the need for labels, self-supervised learning recovers representations of sky survey images that are semantically useful for a variety of scientific tasks. These representations can be directly used as features, or fine-tuned, to outperform supervised methods trained only on labeled data. We apply a contrastive learning framework on multi-band galaxy photometry from the Sloan Digital Sky Survey (SDSS) to learn image representations. We then use them for galaxy morphology classification, and fine-tune them for photometric redshift estimation, using labels from the Galaxy Zoo 2 dataset and SDSS spectroscopy. In both downstream tasks, using the same learned representations, we outperform the supervised state-of-the-art results, and we show that our approach can achieve the accuracy of supervised models while using 2-4 times fewer labels for training.

==> appendices.tex <==
\section{Dataset details}
\label{app:data}

Our database of galaxies is assembled from Data Release 12 (DR12; \citealt{alam2015eleventh}) of the SDSS. To pull samples with spectroscopic redshift labels, we follow the process of \cite{pasquet2019photometric} in pulling from the Main Galaxy Sample to enable direct comparison to their results. Their SQL query filters for objects classified as \texttt{`GALAXY'} with dereddened petrosian magnitudes $r \leq 17.8$ and spectroscopic redshifts $z \leq 0.4$. For us, the query returns 547,224 objects, and after removing some duplicates, we are left with  517,190 to use as labeled training examples. When fine-tuning our image representations for the photo-$z$ estimation task, we use  400,000 images for training and 103,000 as validation dataset.

To build our larger set of galaxies with no spectroscopic labels, we filter for objects with dereddened petrosian magnitudes $r \leq 17.8$, on the \texttt{`PhotoObjAll'} full photometric catalog of the SDSS. In the resulting set of galaxies, we remove duplicates which were already included in our spectroscopic sample, and exclude samples with an estimated photometric redshift (as estimated by \cite{Becketal16photozbaseline}) $z_{phot} > 0.8$. This eliminates objects which are too distant compared to the spectroscopic sample, but decreases the possibility that we are unnecessarily excluding samples whose true redshift is less than 0.4 (the cutoff for our spectroscopic sample) due to incorrect photo-$z$ estimates. After imposing these cuts, we were able to successfully pull 845,254 objects. The spatial distributions of our labeled and unlabeled galaxy datasets are shown in Figure \ref{fig:skymap}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{photoz_dist.pdf}
    \includegraphics[width=0.49\textwidth]{specz_dist.pdf}
    \caption{The spatial distribution of the full unlabeled (left) galaxy image dataset, and the spec-z labeled (right) dataset.}
    \label{fig:skymap}
\end{figure}

SDSS photometric images contain data in 5 passbands ($ugriz$), and come background-subtracted but are not de-reddened to account for galactic extinction. To pull images for our datasets, we use the Montage\footnote{\url{http://montage.ipac.caltech.edu/}} tool to query the imagery catalog in SDSS Data Release 9 (DR9), based on the tabulated equatorial coordinates for each object in our dataset. For each set of object coordinates, we sample a patch of sky of size $(0.012^\circ)^2$, centered on the object, and project onto a 2D image with $107^2$ pixels (this ensures the resulting pixel scale is as close as possible to the native pixel scale in the SDSS, 0.396 arcsec). In each image, we store the $u$, $g$, $r$, $i$, and $z$ passbands as 5 color channels.

The Montage pipeline uses Variable-Pixel Linear Reconstruction \citep{FruchterHook2002VLPR} during the projection process to appropriately transform source input pixel values into the output pixel space. With this setup, a few samples were returned containing corrupted values at the edges of the image, so we crop all images to $107^2$ pixels to eliminate such issues. Note that during training of the self-supervised model, we impose random rotations and random jitter to each image before cropping out the central portion as a data augmentation, so while our photometric images contain 107 pixels per side, the CNNs in this work only view samples of size $64^2$ pixels. This input size of CNN is consistent with the photo-$z$ CNN model of \cite{pasquet2019photometric}.

\section{Galaxy Morphology Classification}\label{app:morphology}
\label{ap:galaxy_morphology}

In Section~\ref{sec:morphology} we displayed morphological predictions for a subset of Galaxy Zoo 2 (GZ2) labels. Here, we describe the training data and detail the training procedure for the linear classifier, and put in further context the accuracy of the predictions with respect to previous methods.

\subsection{Training methodology}
Galaxy Zoo 2 \citep{GZ2} achieved 16 million morphological classifications of 304,122 galaxies drawn from SDSS with r $<$ 17 and petroR90\_r\footnote{petroR90\_r is the Petrosian radius which contains 90\% of the r-band flux} $>$ 3 arcsec, collected via a web-based interface. For each galaxy users were shown a 424$\times$424 pixel image scaled to 0.02petroR90\_r arcseconds per pixel, and were led down a multi-step decision tree to answer increasingly detailed questions about the visual appearance of the galaxy. For example, users were first asked ``Is the galaxy simply smooth and rounded, with no sign of a disk?'', and had the option of selecting responses ``smooth'', ``features or disk'', or ``star or artifact''. Their selection of a response is referred to as their {\textit{vote}}. Based on their response to a question they are lead down different branches of the decision tree - if ``smooth'' was selected, they are next asked ``how rounded is it'', but if ``features or disk'' was selected they will be asked a series of questions about spiral arms, bulge shapes, and a variety of other morphological features.

There are 11 total of these {\textit{classification tasks}} (questions) that have the potential of being asked in the GZ2 decision tree, and the number of possible responses for each classification ranges from 2 to 7. We focus on binary tasks, with the exception of the first question where the response ``star or artifact'' occurs so infrequently (0.08\% of responses select this as the majority) that it can be effectively neglected.  All tasks beyond the first one depend on responses to previous tasks in the decision tree. For example, ``could this be a disk viewed edge on?'' is only asked if the user responded ``features or disk'' on the first task. Thus, a response for ``edge-on'' over ``face-on'' is not a binary classification of the total galaxy population, but only a sub-classification of galaxies that were already considered to have features or a disk.

The nature of data collection (non-expert labelled), coupled with the uncertain class boundaries for galaxies with faint features, result in individual GZ2 users voting for different answers, and therefore uncertain morphological classifications are given for each galaxy. We consider the ``consensus weighted vote fractions'' - the fraction of users who voted for an answer\footnote{consensus weighted fractions are slightly different than the true vote fraction, they are the result of re-weighting users votes based on their overall consensus with others who looked at the same image} -  as the true probability of a galaxy belonging to one class over the other, and we predict an equivalent class probability between (0, 1). Rather than a binary prediction, the returned probability represents the uncertainty of the morphology of the galaxy as seen in an SDSS image, whether this uncertainty stems from faint features, mislabelling, or imaging artifacts. Other works use the ``de-biased estimate'', which estimates how the galaxy would have been classified if viewed at $z=0.03$ \citep{GZ2_debiased}. By using the consensus weighted fractions we estimate what the image actually shows, not the ``true'' morphology, and debiasing can be performed after prediction. 



We use the GZ2 main sample with spectroscopic redshifts which includes morphological classifications for 243,500 galaxies. The main sample without photometric redshifts of 42,462 galaxies, and the stand-alone Stripe 82 catalogue of 17,787 galaxies, were not included. We cross match the GZ2 table\footnote{Galaxy Zoo data is located at \url{https://data.galaxyzoo.org/}} with our SDSS database and search for pairs whose equatorial coordinates overlap within within 5 pixels (1.98 arcsec). This returns a final sample of 183,929 galaxies for which we have both \textit{ugriz} images and crowd-sourced morphological classifications. This sample also contains redshift information which was used separately for photo-z prediction. 

\subsection{Network \& training}
We predict the vote weighted user response by training a simple linear classifier on the self-supervised representations. The linear layer maps the 2048 dimensional representation to 1 dimension with 2048 trainable weights and one bias parameter, followed by a softmax function to ensure the probability is within the range (0, 1). Each GZ2 question has its own linear classifier, trained separately using the subset of galaxies that have at least five total votes for that question. Thus, the predicted probability should be interpreted as follows: regardless of the vote fraction of responses to previous questions, what is the consensus vote {\textit{of the users that ended up at this question on the decision tree}}. If only 10\% of users selected ``features or a disk'' for the first question, the galaxy most likely is smooth and does not have a disk. Yet we still use the vote fraction of that 10\% of users that were then subsequently asked ``could this be a disk viewed edge-on?'' when training a classifier for the edge-on question. Classifiers can then be used in conjunction after training.

Training was conducted in PyTorch~\citep{pytorch} through a binary cross entropy loss on the soft labels (consensus weighted vote fractions). A random sample of 20\% of the data was set aside for testing, and was not used for training any of the classifiers. Many questions have a high degree of class imbalance which reflects the occurrence of galaxy morphologies in the nearby universe. We found that balanced class weights (each instance of the class weighted by the overall occurrence fraction of that class) did not improve the classification performance. Optimization was performed using Limited-memory BFGS (LBFGS) and  a learning rate of 0.01. K-fold cross validation was utilized with $k=5$ by splitting the training dataset into k subsets, training on $k-1$ of them, and using the last as a validation set in order to perform early stopping when the error on the validation set began to increase. Final predictions are then taken as an average over the 5 networks. K-fold cross-validation has no discernible improvement on the results, but was used as it can provide more robust predictions when training with a very small number of labels, and can provide some estimate of uncertainty on the prediction. For each linear classifier, training generally concluded within a few epochs and $\sim 0.5-10$ seconds of compute time on a GPU. Note that this does not take into account the compute time required to learn the self-supervised representations, which this is shared between all downstream tasks, and does not need to be undertaken for each one separately. 

As evidenced by Figure~\ref{fig:umap}, the self-supervised representations have achieved a high degree of separation between numerous types of galaxy morphologies. Likewise, we found that classification became a straightforward task when using any subset of the labels. Unlike DS+18, we found no need to separate uncertain labels from high probability ones. Limiting our training set to only `high quality' (HQ) labels (those with $P<0.2$ or $P>0.8$), resulted in nearly equivalent performance on HQ labels in the test set, but decreased the performance on uncertain labels (those with $0.2 < P < 0.8$). We also found no need to impose higher minimum cuts on the number of votes (10) for some questions, as W+20 found was needed to improve classification performance from random initialization. 

\subsection{Performance metrics \& additional results}

Figure~\ref{fig:morphology} demonstrated the quality of the morphological predictions for three selected GZ2 questions. To measure the performance of a binary classifier, we quantify the accuracy (Acc), Precision (Prec), recall or true positive rate (Rec/TPR), false positive rate (FPR), and area under (AUC) the receiver operator characteristic curve:
\begin{align*}
    \text{Acc} &= \frac{\text{TP} + \text{TN}}{(\text{TP}+\text{FP}) + (\text{TN} + \text{FN})} \\
    \text{Prec} &= \frac{\text{TP}}{\text{TN}+\text{FP}} \\
    \text{Rec/TPR} &= \frac{\text{TP}}{\text{TP}+\text{FN}} \\
    \text{FPR} &= \frac{\text{FP}}{\text{FP}+\text{TN}} \\
    \text{AUC} &= \int \text{TPR} d(\text{FPR}), 
\end{align*}
Where TP and TN are the number of true positives and true negatives, and FP and FN are the number of false positives and false negatives, respectively. Figure~\ref{fig:morphology_appendix} shows these performance metrics in the style of DS+18 figure 4 and W+20 figure 9. The format of Figure~\ref{fig:morphology} was instead displayed in the main text as it displays not just the averaged performance metrics, but illustrates the degree to which each galaxy has been classified correctly, given in some cases very uncertain labels.  

\begin{figure*}
\centering
\includegraphics[width=0.32\linewidth]{question_0.pdf}
\includegraphics[width=0.32\linewidth]{question_1.pdf}
\includegraphics[width=0.32\linewidth]{question_2.pdf}
\caption{Binary classification results for the same three GZ2 questions of Figure~\ref{fig:morphology}, but displayed instead as ROC curves to more easily compare to Figures 4 and 9 from \cite{DS18} and \cite{W20}, respectively. The Precision and TPR are shown as a function of a cut on the predicted probability. Three training set sizes are depicted by the opacity of a line, where training samples were chosen randomly without selecting clean high confidence subsets. Test sets for the three questions are of size (36787, 25531, 20569) for ``All'' and (23740, 20452, 13598) for HQ samples, respectively. Dashed lines show the metrics when applied to all test samples, while solid show when only compared to high quality labels.}
\label{fig:morphology_appendix}
\end{figure*}


We note that an exact quantitative comparison of our performance metrics to these works, or to other automated morphological classification works, is not possible due to a lack of consistency in data sets. The samples used from the full set of GZ2 answers are not consistent: images can be from different SDSS data releases and have inconsistent pixel sizes or number of pixels, they use different observation bands (we use 5 here, while most works use 3), and different GZ2 vote fraction definitions are used as the ``ground truth'' morphological classification. Most importantly, the class imbalance used in training/testing is significantly lower in our work, and more imbalanced datasets will more easily show up as higher metric scores. Nevertheless, the results achieved here are extremely promising, and show that the use self-supervised representations allows us to push beyond the limits of supervised learning for automated morphological classifications. 


Misclassified galaxies have three main failure modes which can be addressed in future work to further improve results beyond those achieved here. Firstly, our images span 25.3 arcseconds, which is not large enough to cover the entire angular extent of very nearby and large galaxies. In contrast, GZ2 participants were shown images scaled to ensure the entire galaxy was always visible, as do other automated classifications. Classifying these limited number of these galaxies is easily achievable by human means, so targeting these few samples is not of top priority. But, for the specific downstream task of classifying galaxy morphologies an additional augmentation which scales the angular extent of galaxies may prove beneficial. Second, a number of misclassified galaxies have imaging artifacts, which fine tuning the network would likely help improve the classification. A similarity search on the  self-supervised representations provides a very valuable tool to isolate these artifacts. Finally, some `misclassified' galaxies are the result of label uncertainty.

%============================================================================

\section{Data augmentation ablation study}\label{app:ablation}
In Section \ref{sec:method} we have listed a basic set of augmentations which make intuitive sense for use in a contrastive learning framework, as each augmentation is associated with some source of observational variability within the images that we want the learned representations to be invariant to. A relevant task in developing the self-supervised model is deciding which combinations of these augmentations are most effective in producing high-quality, semantically useful image representations. This can be answered in a number of ways, but is traditionally done in computer vision by taking a sample downstream task, like image classification, and training a linear classifier on top of the learned representations to perform it. Doing so evaluates the quality of the learned representations by measuring, e.g., how easily different classes are linearly separated in the representation space.

Such an approach is straightforward for the task of morphology classification, but is slightly ill-conceived for something more challenging like photo-z estimation, since the ``classes’’ output by the network represent consecutive redshift bins which should not necessarily be linearly separable. Instead, we evaluate our representations by fine-tuning them for the photo-z estimation task and using the $\sigma_{\rm MAD}$ of predictions on test data as our quality metric. To ensure this metric is more closely tied to the representation quality rather than the supervised fine-tuning process, we only consider the performance of models which are fine-tuned on 10\%, 20\%, and 30\% of the labeled data.

\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{ablation.png}
    \caption{The $\sigma_{\rm MAD}$ of photo-z predictions from models fine-tuned on various fractions of the labeled data, showing how different combinations of augmentations affect downstream performance. Augmentations shown are random rotation (RR), jitter crop (JC), Gaussian noise (GN), galactic reddening (GR), and point spread function (PS).}
    \label{fig:ablation}
\end{figure}

The results of our evaluation are shown in Figure \ref{fig:ablation}. We find that on our dataset, the Gaussian noise augmentation seems to be the strongest, but that the best performance is achieved when we use all augmentations except the PSF smoothing. An important note here is that this finding depends both on our dataset as well as the way we have implemented each augmentation. Using contrastive learning with other surveys would require different implementations and possibly different augmentations, and could produce different ``hierarchies’’ of augmentation strengths. In general, careful thought needs to be put into the data augmentations and which transformations one wants the representations to be invariant against \citep{Xiao2020}.

\section{Additional architecture, hyperparameter, \& training details}
\label{app:architecture}
\subsection{Self-supervised framework}\label{app:encoder}
\textbf{Encoder:} We follow~\citep{he2020momentum, chen2020simple} in using a ResNet50 architecture~\citep{he2016deep} as our encoder. Specifically, we use the implementation of the TorchVision library ({\tt torchvision.models.resnet50}) which is a part of the PyTorch project~\citep{pytorch}. The standard ResNet50, however, is designed to work on wider images than our $64\times64$ ones. To maintain reasonably wide representations by the end of the 50 layers, we change the first {\tt Conv2d} layer to have {\tt stride=1} instead of the default {\tt stride=2}, we also remove the first {\tt MaxPool2d} layer. This gives us $4\times$ wider activations throughout the network than what we would get with the defaults of ResNet50. The output of the {\tt AdaptiveAvgPool2d} layer of the network is our representation, a $2048$ dimensional vector. We also change the number of input channels to 5 to work with our 5 $ugriz$ passbands data.

Following~\citep{chen2020simple,chen2020improved}, we don't use the representation ${\bf {z}}$ directly in the loss in Eq.~\ref{eq:loss}, instead, we use a two layer MLP projection head which maps the representations to a space where the contrastive loss is applied. This has been shown to improve the learned representations. The output of the projection head is a $128$ dimensional vector. The head is discarded after the self-supervised training process is completed.

\textbf{Momentum encoder:} 
In contrastive learning setups, in order to make the task of identifying positive examples non-trivial, it is crucial to have a large set of negative examples. For this we use the momentum encoder idea from~\citep{he2020momentum}; we maintain a queue of size $62$K representations ($\sim 5\%$ of the training dataset size) that is continuously being updated during the training process. The representations in the queue are encoded using a momentum encoder; a second encoder with same architecture whose weights are an exponentially moving average of the main encoder weights. The parameters $\theta_k$ of the momentum encoder network are updated using the encoder parameters $\theta_q$ with momentum parameter $m$ via

\begin{equation}
    \theta_k \leftarrow m\theta_{k}+(1-m)\theta_q. 
\end{equation}

The momentum hyper-parameter is set to $m=0.999$. The momentum encoder helps maintain some consistency between the representations in the negative examples queue during the training. We use temperature parameter $\tau=0.1$ in the contrastive loss.

During self-supervised pre-training, we use stochastic gradient descent with a cosine learning rate schedule, having an initial learning rate of 0.03. We pre-trained our network for 12 hours using 8 NVIDIA V100 GPUs on $\sim$1.2M images to complete $\sim$50 epochs and this proved to be good enough for learning useful features used in this study. We have used \texttt{DistributedDataParallel} of PyTorch to leverage distributed training.

\subsection{Photometric redshift estimation networks}
We closely follow the setup of~\cite{pasquet2019photometric}, whose CNN is trained as a classifier over a discrete set of 180 redshift bins of size $\delta z  = 2.2 \times 10^{-3}$ spanning $0\leq z \leq 0.4$, where the photo-z estimate $z_p$ is computed as the expectation $\mathbb{E}(z)$ over the probabilities predicted in each bin. We train models from scratch to establish a baseline with the ResNet50 architecture (with the same modifications made for the self-supervised pre-training encoder, see~\ref{app:encoder}).  During training, images are de-reddened by using the tabulated $E(B-V)$ value with the photometric calibration in \cite{schlafly2011measuring}, then augmented with random rotations, and random jitter \& crop. Only de-reddening and cropping is applied at testing or evaluation.

For the fine-tuned networks, we take the pre-trained encoder and replace the projection head with a single MLP layer. Here, parameters up to \texttt{AdaptiveAvgPool2d} are initialized with the pre-trained weights and the MLP layer has random initialization. The whole network is then trained on labels, with the pre-trained weights having a learning rate of $0.0001$, and the MLP classifier layer having a learning rate of $0.001$. We train for 100 epochs and reduce the learning rate by a factor of 10 at 60, 90-th epochs.  In all cases we have a batch size of 256.

